Trend Alert: How a Cross-Platform Organization Manipulated Twitter Trends in the Indian General Election

Political organizations worldwide keep innovating their use of social media technologies. In the 2019 Indian general election, organizers used a network of WhatsApp groups to manipulate Twitter trends through coordinated mass postings. We joined 600 WhatsApp groups that support the Bharatiya Janata Party, the right-wing party that won the general election, to investigate these campaigns. We found evidence of 75 hashtag manipulation campaigns in the form of mobilization messages with lists of pre-written tweets. Building on this evidence, we estimate the campaigns' size, describe their organization and determine whether they succeeded in creating controlled social media narratives. Our findings show that the campaigns produced hundreds of nationwide Twitter trends throughout the election. Centrally controlled but voluntary in participation, this hybrid configuration of technologies and organizational strategies shows how profoundly online tools transform campaign politics. Trend alerts complicate the debates over the legitimate use of digital tools for political participation and may have provided a blueprint for participatory media manipulation by a party with popular support.

==> 7_other.tex <==
\section{Conclusion}


\begin{itemize}
	\item  Characterizing coordinated information campaigns on Twitter\par
\end{itemize}

\section{Naming conventions / brainstorming}
\begin{itemize}
	\item  Astroturfing \par

	\item  Template campaigns \par

	\item  Trend alert, tweet bank\par

	\item  "Sample\  Tweet Bank$"$ \par
\end{itemize}




\section{III 1A The WhatsApp messages}

\begin{itemize}
	\item  Qualitative\par

	\item  Evidence that it causes it in any way\par

	\item  How long before the campaign do they come\par

	\item  Do they always say a time\par

	\item  What do they usually say\par

	\item  Tie the story up by how does it start\par

	\item  Are they only doing it on Twitter? Why is it just Twitter?\par

	\item  Always give a time and date when to start\par

	\item  Usually it’s 9am\par

	\item  Do they state the aim of the campaign\par

	\item  How do they try to avoid detection? Look at their explanations, what do they think will help them avoid detection\par
\end{itemize}



%%%%%%%%%%%%%%%%%%%% Figure/Image No: 11 Ends here %%%%%%%%%%%%%%%%%%%%

\section{III.2 Is it effective?}

%%%%%%%%%%%%%%%%%%%% Figure/Image No: 13 Ends here %%%%%%%%%%%%%%%%%%%%

\section{IV. Discussion: }

\begin{itemize}
	\item  We definitely need to note that the rival Congress party is doing the same thing in their Whatsapp groups, maybe with less success

	\item  Effect on other platforms\par

	\item  Will it spill over\par

	\item  Aim\par

    \item most of the stuff discussed was not mis/disinformation. just an infrastructure to spread information. but the same infrastructure can be used to spread propaganda or misinformation. For instance, we observe instances during the 2020 riots in Delhi on the use of such campaigns.
    
    \item Other effects: We also observe that with the success seen by the BJP, many other parties have now started using similar techniques, making it a commonplace political strategy. So it is important to think of information operations in this.
    
    \item in terms of other parties using it, most of them just mention the hashtag and ask to tweet about it. but there are no specific tweets already composed to make it easier to  tweet about it.
    
    \item Every information campaign is inherently coordinated, be it a marketing campaign where there are certain influencers seeding the content or political campaigns where politicians or campaign staff seed them. However, astroturf campaigns are different in that their major seeding structure is a central set of coordinated users 
\cite{walker2014grassroots}.
In many cases, such a central actor might be invisible and their existence could only be hypothesized by looking at particular network properties (e.g. bot like behavior). In our paper, we have clear evidence of the central actor (whatsapp group).

    \item Information operations, especially ones at scale require some collaboration (e.g. GRU activities being coordinated in an office in St. Petersburg). with such collaboration taking place digitally, it is probably easier to identify, especially if we can identify patterns and have better modes of collaboration between platforms. 

    \item It is surprising that Twitter does not detect massive posting of similar content across users. So a small number of unique posts (around 100) can eventually lead to conversations which are around 100k tweets.
    
    \item this level of national coordination is not a trivial thing as India is quite diverse in terms of linguistic and cultural identities. We see successful manipulated campaigns from all over India from the north to the south in multiple languages.
    
    \item These hashtags may not just be political. Given the complex infrastructure setup, hashtags that target individuals from the minority community (e.g. \#ArrestTahirHussain) or boycotting movies that show hindus in a negative light (\#BoycottChhappak) or \#LoveJihadIsAReality (dog whistling against inter religious marriage).
    
    \item Future work: We do not analyze the use of images in this paper. Though most campaigns do have a set of curated images as well. It would be interesting to look at those and their spread across platforms.

	\item  Trending topics\par

	\item  These information operations are collaborative work\par

	\item  They are not easy to detect for users, bot detection fails, but there are algorithmic ways to diagnose them still\par

	\item  Their extent is major and they have significant effects, is this acceptable?\par
	
	\item Not just a BJP thing. They pioneered the scale. We see recent examples from other parties. Congress (INC) has their techniques but they dont seem to be that effective. or at a much smaller scale\footnote{from what we've noticed it is usually done through the twitter account \url{https://twitter.com/trend4india}}

	\item  "Just advertising 101$"$  – standard marketing practice\par

	\item  The party doesn’t try hard to hide their actions, they’re even proud\par

	\item  The more liquid and organic nature of participation makes it hard to take measures\par

	\item  The responsibility of the platform\par

	\item  This clearly breaks Twitters’ policies\par

	\item  Do we see any actions taken? (Deleted users?)\par

	\item  It’s part of the BJP’s massive social media campaigns that may have helped them to power for the second time\par

	\item  Active actions is difficult and costly ("plausible deniability$"$ )\par

	\item  But it would be cheap to make their trending system resistant to such campaigns using our algorithm\par

	\item  None of this is clearly immoral\par

	\item  Little of what people say in their daily lives is original\par

	\item  And much is an echo of what others said before\par

	\item  Is there an obligation of any kind to disclose that your tweet is not your invention?\par

	\item  Not really. Very few areas of life, such as academia, know such obligations, and even there it is difficult.\par

	\item  Furthermore, the agents themselves do not see it as problematic. In most cases they don’t try to hide their traces. They are explicit about what they’re doing and even boast about it.\par

	\item  However, all of this clearly violates Twitter’s policies. But the violation doesn’t seem bad enough for Twitter to do much about it, even if it was technically feasible and inexpensive.\par

	\item  Share campaign tweet IDs, provide this data in some way

	\item  Connect it to CSCW lit: \par

	\item  Kate Starbird\par

	\item  Justin Cheng, Collective action\par

	\item  Matt Salganik – Twitter as exhaust pipe, trails that are left behind that we can study\par
	
\end{itemize}



\begin{itemize}
	\item  Data acquisition \cite{garimella2018whatsapp}

	\item  Data cleaning and preparation\par

	\item  Consolidation of campaigns: Where do we have reliable data?\par

	\item  We did not do image-based matching, and we might not have complete view of the documents used\par

	\item  Identify potential template documents – which tweets, based on the steps described in XX, might have been results of coordination?\par

	\item  Only use campaigns where we can match at least 80$\%$  of suspicious tweets with our data sets\par

	\item   Only campaigns where we matched more than 50 original tweets with our template documents.\par

	\item  Resulting in 25 campaigns, they are all BJP\par

	\item  Main takeaways\par

	\item  Definition and thick description of templating in the case of the BJP\par

	\item  Develop a way to detect campaign programmatically\par

	\item  Show the prevalence, effectiveness, and Twitter’s inaction\par
\end{itemize}


